Human-level Atari 200x faster

The task of building general agents that perform well over a wide range of tasks has been an important goal in reinforcement learning since its inception. The problem has been subject of research of a large body of work, with performance frequently measured by observing scores over the wide range of environments contained in the Atari 57 benchmark. Agent57 was the first agent to surpass the human benchmark on all 57 games, but this came at the cost of poor data-efficiency, requiring nearly 80 billion frames of experience to achieve. Taking Agent57 as a starting point, we employ a diverse set of strategies to achieve a 200-fold reduction of experience needed to out perform the human baseline. We investigate a range of instabilities and bottlenecks we encountered while reducing the data regime, and propose effective solutions to build a more robust and efficient agent. We also demonstrate competitive performance with high-performing methods such as Muesli and MuZero. The four key components to our approach are (1) an approximate trust region method which enables stable bootstrapping from the online network, (2) a normalisation scheme for the loss and priorities which improves robustness when learning a set of value functions with a wide range of scales, (3) an improved architecture employing techniques from NFNets in order to leverage deeper networks without the need for normalization layers, and (4) a policy distillation method which serves to smooth out the instantaneous greedy policy overtime.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

\DeclareMathOperator{\greedy}{\mathcal{G}}
\DeclareMathOperator{\epsgreedy}{\mathcal{G}_{\epsilon}}
\DeclareMathOperator{\pilambda}{\pi_{\lambda}}
\DeclareMathOperator{\pingu}{\pi_{\text{NGU}}}

% Remove horizontal space, useful for large tables
\newcommand{\nsp}{\hspace{-1mm}}

% Highlight TODO's in red
\def\todo#1{\textcolor{red}{TODO: #1}}
\def\p#1{\textcolor{blue}{P: #1}}


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/method_old.tex <==
\newcommand{\sgn}{\operatorname{sgn}}

\section{Super-charging Sample-efficiency in Agent57}
\label{section:methods}

This section describes our main algorithmic contributions to improve the data efficiency of Agent57, grouped by the type of limitation they target.

\subsection{Differing Value Function Scales}
\label{value_scales}

\noindent\textbf{Loss and Priority Normalization.} As we learn a family of Q-functions which vary over a wide range of discount factors and intrinsic reward scales, we expect that the Q-functions will vary considerably in scale. This may cause the larger scale Q-values to dominate learning and destabilize learning of smaller Q-values. This is a particular concern in environments with very small extrinsic reward scales.
%
To counteract this effect we introduce a normalization scheme on the TD-errors similar to that used in \citet{schaul2021return}. Specifically, we compute a running estimate of the standard deviation of TD-errors of the online network $\sigma_i^{running}$ and divide the current TD-errors by the max of this running estimate and the batch standard deviation $\sigma_i^{batch}$. We also bound the standard deviation by a small $\epsilon$ to avoid amplification of noise past a specified scale to get $\sigma_i = \max(\sigma_i^{running}, \sigma_i^{batch}, \epsilon)$, where $\epsilon=0.01$ in all our experiments.
%
% \begin{equation}
%     \sigma_i = \max(\sigma_i^{running}, \sigma_i^{batch}, \epsilon)
% \end{equation}
%
In order to fully remove the instability it is necessary to apply this normalization to the TD-errors in both the loss and priorities.


\noindent\textbf{Cross-mixture training.}
Agent57 only trains the policy which collected a given trajectory, but it is natural to ask whether data-efficiency and robustness may be improved by training all policies at once. To achieve better compute-efficiency we choose to deviate from the original UVFA architecture which fed a 1-hot encoding of the policy index to the LSTM, and instead modify the dueling head to output values for all combinations of actions and policies. We consider the following weighting scheme between the behavior policy loss and the mean over all losses:
\begin{equation}
    L = \sum_{i=1}^N \bigg(\eta L_i \mathbb{I}_{\left[i = i_{behavior} \right]} + \frac{1-\eta}{N} L_i\bigg)
\end{equation}
where $L_i$ denotes the RL loss for policy $i$. We find that an intermediate value of $\eta=0.5$ tends to work well. Critically, we only observe a significant improvement when using this method in conjunction with our TD-normalization scheme.

\subsection{Signal Propagation of Rare Events}
\label{sec:signal_propagation_of_rare_events}

\noindent\textbf{Bootstrapping with online network.}
Target networks are frequently used in conjunction with value based agents due to their stabilizing effect when learning from off-policy data. The cost of this design choice is a fundamental restriction on how quickly changes in the Q-function are able to propagate. This issue can be mitigated to some extent by simply updating the target network more frequently, but the result is typically a less stable agent.
%
% To stabilise the learning with online network bootstrapping, we introduce a trust region for value updates that allows us to filter which samples contribute to the loss.
%
To accelerate signal propagation, we use online network bootstrapping, and we stabilise the learning by introducing a trust region for value updates that allows us to filter which samples contribute to the loss.
%
The trust region masks the loss at any timestep for which \textit{both} of the following conditions hold: 
\begin{align}
\label{eq_tr_1}
    |Q_i(x_t, a_t) - Q_i^T(x_t, a_t)| &> \beta_{std} \sigma_i \\
\label{eq_tr_2}
    \sgn(Q_i(x_t, a_t) - \widehat{Q}_i(x_t, a_t) &\neq \sgn(Q_i(x_t, a_t) - Q_i^T(x_t, a_t))
\end{align}
where $\beta_{std}$ is a fixed hyperparameter, $\widehat{Q_i}(x_t, a_t)$ denotes the return estimate, $\sigma_i$ is the standard deviation of the TD-errors as in Sec. \ref{value_scales}, and $\sgn$ is the sign function. Intuitively, we only mask if \textit{the current value of the online network is outside of the trust region} (Eq. \ref{eq_tr_1}) and \textit{the TD-error points away from the trust region} (Eq. \ref{eq_tr_2}). We note that a very similar trust region scheme is used for the value-function in most PPO implementations~\citep{schulman2017proximal}, though not described in the original paper. The PPO version instead uses a constant threshold, and thus is not able to adapt to differing scales of value functions.

\noindent\textbf{Target computation with tolerance.}
Watkins Q($\lambda$) may cut the traces too aggressively as soon as an action is considered to be off-policy, and thus lose information.
To relax this issue, we introduce a relative tolerance when estimating the difference between Q-values used to compute the $\lambda$ parameter for trace cutting:
\begin{equation}
\label{eq_soft_watkins}
    \lambda_t = \lambda 
    \left ( 
        \sum_{a'} \pi (a'|s_t) \mathbb{I}_{
            \left [ Q(a_t, s_t) \leq Q(a', s_t) - \kappa \left | Q(a', s_t) \right | \right ]
            } 
    \right )
\end{equation}
This \textit{Soft Watkins Q($\lambda$)} approach leads to more transitions being used, and thus increases sample efficiency. Note that Watkins Q($\lambda$) is recovered when setting the tolerance parameter $\kappa = 0$.

% \noindent\textbf{Stabilising high replay ratios.}
% The \textit{replay ratio} is defined as the ratio of learner samples to actor inserts. Increasing the replay ratio might seem a straightforward way to improve the sample efficiency of an agent, but this can cause instabilities if set too high, and may additionally incur a cost in wall-clock time depending on the resources used.

\subsection{Building a Better Network}

% \subsubsection{Normalizer-free Torso Network.}
% We have increased the expressive power of the value function approximator, by implementing a ResNet-style torso network as opposed to a simple ConvNet. Based on findings from prior work \textcolor{red}{\citep{brock2021high}} and ablation experiments \textcolor{red}{(Fig.~\ref{fig:ablations_better_network})}, we concluded that applying normalisation actually hurts performance. Therefore, we implement NFNet-style torso to achieve greater learning stability.


\noindent\textbf{Normalizer-free Torso Network.} Normalization layers are a common feature of ResNet architectures which are known to aid in training of very deep networks, but our investigation revealed that several commonly used normalization layers are in fact detrimental to performance in our setting. Instead, we employ a variation of the NFNet architecture~\citep{brock2021high} for our policy torso network, which combines a variance-scaling strategy with scaled weight standardization and careful initialization to achieve state-of-the-art performance on ImageNet without the need for normalization layers. We adopt their use of stochastic depth~\citep{huang2016deep} but omitted the application of ordinary dropout to fully-connected layers as we did not observe any benefit from this form of regularization.
%
The implementation of stochastic depth in conjunction with multi-step returns requires some care, as resampling the stochastic depth mask at each timestep can serve to inject additional noise into our bootstrap values, resulting in a higher variance return estimator. As such, we use a \textit{temporally-consistent} stochastic depth mask which remains fixed over the length of each training trajectory.

\noindent\textbf{Shared torso with Combined Loss.}
Agent57 decomposes the combined Q-function into intrinsic and extrinsic components which are represented by separate networks. 
%
Such decomposition prevents the gradients of the decomposed value functions from interfering with each other. This may occur in environments where the intrinsic reward is poorly aligned with the task objective, as defined by the extrinsic reward, while still ensuring convergence to $Q^\star$ in the tabular setting.
%
However, this is incorrect when using function approximation with shared parameters and decomposed losses, as we observe a mismatch in gradients between these two variants:
%However, the story is not so clean with function approximation, as we observe a mismatch in gradients between these two variants:
\begin{equation}
    % \frac{\partial}{\partial \Theta} \Big[\frac{1}{2}(Q_{ext}(\Theta) + \beta Q_{int}(\Theta) - \hat{Q})^2 \Big]
    {\underbrace{\textstyle \frac{\partial}{\partial \Theta} \Big[\frac{1}{2}(Q_{\text{ext}}(\Theta) + \beta Q_{\text{int}}(\Theta) - \hat{Q})^2 \Big]}_{\mathclap{\text{combined loss}}}}
    \neq
    % \frac{\partial}{\partial \Theta} \Big[ \frac{1}{2}(Q_{ext}(\Theta) - \hat{Q_{ext}})^2 + \frac{1}{2}(Q_{int}(\Theta) - \hat{Q_{int}})^2 \Big]
    {\underbrace{\textstyle \frac{\partial}{\partial \Theta} \Big[ \frac{1}{2}(Q_{\text{ext}}(\Theta) - \hat{Q}_{\text{ext}})^2 + \frac{1}{2}(Q_{\text{int}}(\Theta) - \hat{Q}_{\text{int}})^2 \Big]}_{\mathclap{\text{decomposed loss}}}}
\end{equation}
% $$\frac{\partial}{\partial \Theta} \Big[\frac{1}{2}(Q_{ext}(\Theta) + \beta Q_{int}(\Theta) - \hat{Q})^2 \Big]
% \neq \frac{\partial}{\partial \Theta} \Big[ \frac{1}{2}(Q_{ext}(\Theta) - \hat{Q_{ext}})^2 + \frac{1}{2}(Q_{int}(\Theta) - \hat{Q_{int}})^2 \Big]$$ 

Since we always use a behavior policy induced by the total Q-function rather than the individual components, theory would suggest to  use the combined loss instead. In addition, from a practical implementation perspective, this switch to the combined loss greatly simplifies the design choices involved in our proposed trust region method.
%
The penalty paid for this choice is that the decomposition of the value function into extrinsic and intrinsic components no longer carries a strict semantic meaning. Nevertheless we do still retain an implicit inductive bias induced by multiplication with the intrinsic reward weight, $\beta$. 

% For computational efficiency it is also desirable to merge th

% \subsection{Robustifying Behavior via Policy Distillation.}
% \citet{schaul2022phenomenon} describe the effect of policy churn, whereby the greedy action of value-based RL algorithms may change frequently over consecutive parameter updates. This can have a deleterious effect on off-policy correction methods: traces will be cut more aggressively than a policy which is smoothed over time, causing the bootstrap value to change frequently and resulting in a higher variance return estimator. 
% By utilizing an additional policy head trained via policy distillation we can obtain a more stable return estimator, which provides substantial improvement in sparse-reward environments such as Pitfall.

% Our choice of training with temporally-consistent stochastic depth masks can be interpreted as learning an implicit ensemble of Q-functions, thus it is natural to ask whether we may see additional benefit from utilizing the policy induced by this ensemble.
% Prior work found that applying a majority voting scheme as the behavior policy for an ensemble of Q-functions yielded significant gains over vanilla DQN~\citep{osband2016deep}. In our case, each member of the ensemble is expensive to compute as it would require an additional forward pass of the full network, and many samples may be required to obtain a good approximation of the true majority action, rendering an explicit computation intractable.

% To overcome both of these obstacles we propose to leverage a policy head $\pi_{dist}$ trained via policy distillation to match the $\epsilon$-Greedy policy induced by the Q-function; in effect, smoothing out the policy over time, as well as over the ensemble. We also include a KL constraint $C_{\text{KL}}$ between the online and target policies, and mask $L_{\pi}$ at any timestep where this is violated.
% \begin{equation}
%     L_{\pi} = -\sum_{a} \pi_{\epsilon-\text{Greedy}}(Q)(a) log(\pi_{\text{dist}}(a))
% \end{equation}
% \begin{equation}
%     KL(\pi^T_{\text{dist}}(a)) || \pi_{\text{dist}}(a))) \le C_{KL}
% \end{equation}

\subsection{Robustifying Behavior via Policy Distillation}
\citet{schaul2022phenomenon} describe the effect of policy churn, whereby the greedy action of value-based RL algorithms may change frequently over consecutive parameter updates. This can have a deleterious effect on off-policy correction methods: traces will be cut more aggressively than a policy which is smoothed over time, causing the bootstrap value to change frequently and resulting in a higher variance return estimator.
Our choice of training with temporally-consistent stochastic depth masks can be interpreted as learning an implicit ensemble of Q-functions, thus it is natural to ask whether we may see additional benefit from utilizing the policy induced by this ensemble. We propose to leverage a policy head $\pi_{\mathrm{dist}}$ trained via policy distillation to match the $\epsilon$-Greedy policy induced by the Q-function. This decreases policy churn by smoothing out the policy over time, as well as over the ensemble, while being much faster to evaluate than the members of the ensemble. Similarly to the trust-region described in Section~\ref{sec:signal_propagation_of_rare_events}, we mask the policy distillation loss at any timestep where a KL constraint $C_{\text{KL}}$ is violated:
\begin{equation}
    L_{\pi} = -\sum_{a,t} \pi_{\epsilon-\text{Greedy}}(Q)(x_t, a) log(\pi_{\text{dist}}(x_t, a)) \quad\quad
    \forall t \ni KL(\pi^T_{\text{dist}}(x_t, a)) || \pi_{\text{dist}}(x_t, a))) \le C_{\text{KL}}
\end{equation}
%where $\pi^T_{\text{dist}}$ is the distilled policy estimated
We use $\pi_{\mathrm{dist}}$ as the target policy when computing bootstrap values in the return estimator, $V(x_t) = \sum_a \pi_{\mathrm{dist}}(a_t) Q(x_t, a_T)$, but found that sampling from the distilled policy at behavior-time was less effective in some sparse reward environments. In analogy to the majority-voting scheme used in previous works~\citep{osband2016deep}, we instead opt to have the agent act according to $\arg\!\max(\pi_{\mathrm{dist}})$.

% We use $\pi_{\text{dist}}$ as the target policy when computing bootstrap values in the return estimator, $V(x_t) = \sum_a \pi_{\text{dist}}(a_t) Q(x_t, a_T)$, but found that sampling from the distilled policy at behavior-time was less effective in some sparse reward environments. In analogy to majority-voting, we instead opt to have the agent act according to $\arg\!\max(\pi_{\text{dist}})$.

